Formal Semantics of Heterogeneous CUDA-C: A Modular Approach with Applications

We extend an off-the-shelf, executable formal semantics of C (Ellison and Rosu's K Framework semantics) with the core features of CUDA-C. The hybrid CPU/GPU computation model of CUDA-C presents challenges not just for programmers, but also for practitioners of formal methods. Our formal semantics helps expose and clarify these issues. We demonstrate the usefulness of our semantics by generating a tool from it capable of detecting some race conditions and deadlocks in CUDA-C programs. We discuss limitations of our model and argue that its extensibility can easily enable a wider range of verification tasks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{115}
\providecommand{\publicationstatus}{F. Cassez, R. Huuck, G. Klein and B. Schlich (eds.):\\ Systems Software Verification Conference 2012 (SSV 2012)\\
EPTCS 102, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.102.11}{10.4204/EPTCS.102.11}}

